Generating Data to Mitigate Spurious Correlations in Natural Language Inference Datasets

Natural language processing models often exploit spurious correlations between task-independent features and labels in datasets to perform well only within the distributions they are trained on, while not generalising to different task distributions. We propose to tackle this problem by generating a debiased version of a dataset, which can then be used to train a debiased, off-the-shelf model, by simply replacing its training data. Our approach consists of 1) a method for training data generators to generate high-quality, label-consistent data samples; and 2) a filtering mechanism for removing data points that contribute to spurious correlations, measured in terms of z-statistics. We generate debiased versions of the SNLI and MNLI datasets, and we evaluate on a large suite of debiased, out-of-distribution, and adversarial test sets. Results show that models trained on our debiased datasets generalise better than those trained on the original datasets in all settings. On the majority of the datasets, our method outperforms or performs comparably to previous state-of-the-art debiasing strategies, and when combined with an orthogonal technique, product-of-experts, it improves further and outperforms previous best results of SNLI-hard and MNLI-hard.

==> analysis.tex <==
\section{Analysis} \label{sec:analysis}






==> related.tex <==
\newacronym{poe}{PoE}{Product-of-Expert}

\section{Related Work}

% Annotation artifacts (not just NLI)
\paragraph{Annotation Artifacts.}
% 
Annotation artifacts (or dataset biases) are commonly-observed in a wide range of crowdsourced datasets~\citep{zeichner2012crowdsourcing,sick,cnndailymail,vqa,squad}.
%
This is an inherent problem of data annotation, often caused by biases of the task framing~\citep{schwartz-etal-2017-effect}, noisy annotations~\citep{chen-etal-2016-thorough}, or the group biases of the annotators~\citep{liu2021toward}.
% Gender biases: \citep{mitigate-gender-biases,quantify-stereotype-in-plm}

\paragraph{Artifacts in \ourtask{}.}
Previous works~\citep{GururanganSLSBS18,PoliakNHRD18} found that models leverage dataset artifacts in SNLI~\citep{snli} and MNLI~\citep{mnli} to achieve high performances while failing to generalize to out-of-distribution test sets. 
% evaluation data
To tackle the hypothesis-only biases in NLI, \citet{GururanganSLSBS18} proposed a harder (out-of-distribution) in-domain test set SNLI-hard, and later \citet{PoliakNHRD18} chose some out-of-domain datasets and recasted them for NLI evaluation.
% HANS (lexical overlap)
\cite{hans} introduced a evaluation set HANS that contains examples where syntactic heuristics will fail.
More recently, \citet{model-agnostic-debias} proposed an aggregated benchmark consisted of a suite of adversarial datasets, each testing a different aspect of robustness of the NLI models.
% Gender-biases NLI \cite{gender-nli}
% FEVER

% Identifying or quantifying biases: z-score

\paragraph{Debiasing NLI Models.}
%
Constructing unbiased datasets, especially at large scale, is costly and challenging. Therefore, most previous works follow a \emph{model-centric} approach towards mitigating biases in NLI models -- they propose novel model architectures or training objectives to debias the model.
% 
At representation level, \citet{belinkov-etal-2019-dont,belinkov-etal-2019-adversarial} introduce an adversarial architecture to debias hypothesis representations to tackle the hypothesis-only bias, and \citet{stacey-etal-2020-avoiding} strengthen the debiasing with multiple adversarial classifiers.
\citet{zhou-bansal-2020-towards} use HEX projection to project the representation to the space orthogonal to the biased features.
% model-level
At model level, \citet{clark-etal-2019-dont,he-etal-2019-unlearn,karimi-mahabadi-etal-2020-end} propose to use \acrfull{poe} for mitigating biases. % and \citet{karimi-mahabadi-etal-2020-end} propose an end-to-end variant of \acrshort{poe}. 
\citet{utama-etal-2020-mind} propose confidence regularization to improve out-of-distribution performance while retaining in-distribution accuracy. 
% weakness of model-centric approach
These methods require changing the model architecture or the learning objective of the model, and often lead to a more complex training procedure.

\paragraph{Debiasing \ourtask{} Datasets.}
%
To avoid the high cost of manually curating unbiased datasets, some previous works explored data augmentation with heuristics. \citet{zhou-bansal-2020-towards} appended meaningless sentences at the end of the hypothesis to create new samples, and repeated some samples to debias word-overlap bias and contradiction word bias, but they fail to get performance gains. \citet{ross2021tailor} introduce TAILOR, a semantically-controlled perturbation method for data augmentation, but it still requires labeling heuristics and is not targeted to debias annotation artifacts. The closest work to our is CrossAug~\citet{lee2021crossaug} that learns a BART data generator to generate new claims and evidences for debiasing fact verification models. However, it requires an external training dataset that provides pairs of positive claims and their corresponding negative claims, which is not available in other \ourtask{} tasks.

% Data augmentation / data generation 
\paragraph{Data Augmentation in NLP} 
% % Previous work mainly adopts heuristics (or templates) to conduct data augmentation. Some works use a paraphrasing system to generate semantically equivalent instances.
% % 
With the surge of pretrained language models, some recent works start to exploit PLMs to conduct data augmentation. 
% 
To the best of our knowledge, our work is the first to exploit PLM to debias a dataset. 
% 
\citet{bartolo2021improving} propose to generate adversarial data for improving QA model robustness.

% Our novelty: start with a biased dataset, exploit PLM to debias a dataset.

